Joint Local Relational Augmentation and Global Nash Equilibrium for Federated Learning with Non-IID Data

Federated learning (FL) is a distributed machine learning paradigm that needs collaboration between a server and a series of clients with decentralized data. To make FL effective in real-world applications, existing work devotes to improving the modeling of decentralized data with non-independent and identical distributions (non-IID). In non-IID settings, there are intra-client inconsistency that comes from the imbalanced data modeling, and inter-client inconsistency among heterogeneous client distributions, which not only hinders sufficient representation of the minority data, but also brings discrepant model deviations. However, previous work overlooks to tackle the above two coupling inconsistencies together. In this work, we propose FedRANE, which consists of two main modules, i.e., local relational augmentation (LRA) and global Nash equilibrium (GNE), to resolve intra- and inter-client inconsistency simultaneously. Specifically, in each client, LRA mines the similarity relations among different data samples and enhances the minority sample representations with their neighbors using attentive message passing. In server, GNE reaches an agreement among inconsistent and discrepant model deviations from clients to server, which encourages the global model to update in the direction of global optimum without breaking down the clients optimization toward their local optimums. We conduct extensive experiments on four benchmark datasets to show the superiority of FedRANE in enhancing the performance of FL with non-IID data.

==> chapter/preliminaries.tex <==
\section{Preliminaries}

\subsection{Poincar\'e ball model}
% 用自己的话表达 Hyperbolic Image Segmentation
% ref Hyperbolic visual embedding learning for zero-shot recognition
Poincar\'e ball model is one of the common models in hyperbolic space, which is a type of Riemannian manifold $\mathcal{M}$ with constant negative curvature.
%
In this work, $||\boldsymbol{x}||_2 = \sqrt{\Sigma_{i=1}^n x_i^2}$ is a Euclidean norm.
% 
The Poincar\'e is an open ball model in $n$-dimensional hyperbolic space defined as $(\mathbb{P}^n, g^{\mathbb{P}})$, where $\mathbb{P}^n = \{\boldsymbol{x}\in \mathbb{R}^n: ||\boldsymbol{x}||_2 < 1\}$ 
and $g^{\mathbb{P}}$ is the Riemannian metric of a Poincar\'e ball.
% 
$g^{\mathbb{P}}$ is conformal to the metric of Euclidean space $g^\mathbb{E}$, i.e.,
$
g^{\mathbb{P}}_{\boldsymbol{x}} = \lambda_{\boldsymbol{x}}^2 g^\mathbb{E},
$
where $\lambda_{\boldsymbol{x}}=\frac{2}{1-||\boldsymbol{x}||_2^2}$ is the conformer factor.
% \xenia{and $g^\mathbb{E}$ is the metric of Euclidean space}.
%
Given two points in the Poincar\'e ball model, i.e., $\boldsymbol{x}_1, \boldsymbol{x}_2\in \mathbb{P}^n$, the M\"obious addition is defined as:
$$\boldsymbol{x}_1\oplus \boldsymbol{x}_2 = \frac{(1+2\langle\boldsymbol{x}_1, \boldsymbol{x}_2\rangle + ||\boldsymbol{x}_2||_2^2)\boldsymbol{x}_1 +(1-||\boldsymbol{x}_1||_2)\boldsymbol{x}_2^2}{1+2\langle\boldsymbol{x}_1, \boldsymbol{x}_2\rangle + ||\boldsymbol{x}_1||_2^2||\boldsymbol{x}_2||_2^2 }$$
%
We can define the geodesic distance, i.e., the shortest distance between these two points in the Poincar\'e ball, i.e., $\boldsymbol{x}_1, \boldsymbol{x}_2\in \mathbb{P}^n$ as below:
\begin{equation}\label{eq:geo_dis}
    d(\boldsymbol{x}_1, \boldsymbol{x}_2) = \operatorname{arcosh}(1 + \frac{2||\boldsymbol{x}_1-\boldsymbol{x}_2||_2^2}{(1 -  ||\boldsymbol{x}_1||_2^2)(1 - ||\boldsymbol{x}_2||_2^2)}).
\end{equation}
%
%
For a point $\boldsymbol{x}$ in a manifold $\mathcal{M}$, the tangent space $T_{\boldsymbol{x}} \mathcal{M}$ is a vector space comprising all directions that are tangent to $\mathcal{M}$ at $\boldsymbol{x}$.
% \xenia{For a point $x$ in a manifold $\mathcal{M}$, one can define the tangent space $T_x \mathcal{M}$ of $\mathcal{M}$ at $x$ as a vector space that contains all possible directions in which one can tangentially pass through. An inner product can be defined on $T_x \mathcal{M}$. }
% 
Exponential map $\exp_{\boldsymbol{x}}: T_{\boldsymbol{x}} \mathcal{M} \rightarrow \mathcal{M}$ is a map to 
project any point $\boldsymbol{u}$ from the Euclidean tangent space to the Poincar\'e ball referred by point $\boldsymbol{x}$, defined as below:
\begin{equation}
\exp _{\boldsymbol{x}}(\boldsymbol{u})=\boldsymbol{x} \oplus\left(\tanh \left(\frac{\lambda_{\boldsymbol{x}}\|\boldsymbol{u}\|_2}{2}\right) \frac{\boldsymbol{u}}{\|\boldsymbol{u}\|_2}\right).
\end{equation}
%
The reverse process is logarithmic map, i.e., $\log _{\boldsymbol{x}}(\boldsymbol{y}): \mathcal{M} \rightarrow T_{\mathbf{x}} \mathcal{M}$, which projects hyperbolic vector back to Euclidean space.
% 
% %
\subsection{Riemannian Stochastic Gradient Descent}
In Euclidean space, the Stochastic Gradient Descent (SGD) algorithm for optimizing an objective loss function $\mathcal{L}$ is:
%
\begin{equation}\label{eq:SGD}
\boldsymbol{\theta}^{t+1} = \boldsymbol{\theta}^t - \eta \nabla\mathcal{L},     
\end{equation}
%
where $\boldsymbol{\theta}^t$ represents the parameters at iteration step $t$, $\eta$ is the learning rate and $\nabla\mathcal{L}$ is the Euclidean gradient of the loss function.
%
To generalize to a Riemannian manifold $\mathcal{M}$, \cite{bonnabel2013stochastic} propose the Riemannian Stochastic Gradient Descent(RSGD), which is defined as:
%
\begin{equation} \label{eq:RSGD}    
\boldsymbol{\theta}^{t+1} = \exp_{\boldsymbol{\theta}^t}(-\eta\nabla_R\mathcal{L}).
\end{equation}
%
In Poincar\'e ball model, the Riemannian gradient $\nabla_R\mathcal{L} = (g^{\mathbb{P}}_{\boldsymbol{\theta}^t})^{-1}\nabla \mathcal{L}$ is obtained by rescaling the Euclidean gradient with the inverse of the Poincar\'e ball metric tensor. 
%
It is noticeable that Euclidean space is the 0-curvature manifold, i.e., $\exp_{\boldsymbol{x}}(\boldsymbol{u})=\boldsymbol{x} + \boldsymbol{u}$, at which Eq.~\eqref{eq:SGD} and Eq.~\eqref{eq:RSGD} are identical.


% To find the optimal solution of a loss function $\mathcal{L}: \mathbb{P}^n\rightarrow \mathbb{R}$ with parameters $\boldsymbol{\theta}$, the Rienmannian Stochastic Gradient Descent is defined as 
% \begin{equation} \label{eq:RSGD}    
% \boldsymbol{\theta}^{t+1} = \exp_{\boldsymbol{\theta}}(-\eta_t\nabla_R\mathcal{L})
% \end{equation}
% ~\cite{bonnabel2013stochastic},
% %
% where $\eta$ is the learning rate and $\nabla_R \mathcal{L}=((\lambda_{\boldsymbol{x}})^2 \mathbb{I}^n)^{-1} \nabla\mathcal{L}$ is the Riemannian gradient.



